Evaluation of QAOA based on the approximation ratio of individual samples

The Quantum Approximate Optimization Algorithm (QAOA) is a hybrid quantum-classical algorithm to solve binary-variable optimization problems. Due to the short circuit depth and its expected robustness to systematic errors, it is one of the promising candidates likely to run on near-term quantum devices. We simulate the performance of QAOA applied to the Max-Cut problem and compare it with some of the best classical alternatives, for exact, approximate and heuristic solution. When comparing solvers, their performance is characterized by the computational time taken to achieve a given quality of solution. Since QAOA is based on sampling, we utilize performance metrics based on the probability of observing a sample above a certain quality. In addition, we show that the QAOA performance varies significantly with the graph type. By selecting a suitable optimizer for the variational parameters and reducing the number of function evaluations, QAOA performance improves by up to 2 orders of magnitude compared to previous estimates. Especially for 3-regular random graphs, this setting decreases the performance gap with classical alternatives. Because of the evolving QAOA computational complexity-theoretic guidance, we utilize a framework for the search for quantum advantage which incorporates a large number of problem instances and all three classical solver modalities: exact, approximate, and heuristic.

==> extra-material.tex <==
%------------------------------------------------------------------
\section{Extra material}
\label{sec:extra}
%------------------------------------------------------------------

\note{probably excluded from this work}

What about \textbf{quantum SDP-solver} algorithms?
\begin{itemize}
    \item Quantum SDP Solvers: Large Speed-ups, Optimality, and Applications to Quantum Learning\cite{brandao_quantum_2017}
    \item Improvements in Quantum SDP-Solving wit applications \cite{van_apeldoorn_improvements_2018}
    \item Quantum-inspired classical sublinear-time algorithm for solving low-rank semidefinite programming via sampling approaches \cite{chia_quantum-inspired_2019}
\end{itemize}

Possibility of a quantum version of MBO?


==> general-considerations-on-QAOA.tex <==
%------------------------------------------------------------------
\subsection{Sampling equations for QAOA}
%------------------------------------------------------------------

\begin{equation}
    \underset{\theta}{min} E(\theta) = \left\langle \Psi(\theta) | \hat{H} | \Psi(\theta) \right\langle
\end{equation}

\begin{equation}
    \hat{H} = \sum_i \alpha_i \hat{P_i} 
\end{equation}

\begin{equation}
    \left\langle \Psi(\theta) | \hat{H} | \Psi(\theta) \right\rangle = \sum_i \alpha_i \left\langle \Psi(\theta) | \hat{P_i} | \Psi(\theta) \right\rangle
\end{equation}

Even with perfect fidelity, each of these expectations is estimated by 
sampling the output of the quantum computer.  

\begin{equation}\label{eq:hamiltonian}
    \hat{h}_{j} = \sum_{i=1}^{j} \alpha_i \hat{P_i} 
\end{equation}

To estimate the expectation value $\left\langle \hat{h}_{j} \right\rangle$ within an accuracy $\epsilon$:

\begin{equation}
    samples \propto \mathcal{O}(\left\Vert \hat{h}_{j} \right\Vert^2/ \epsilon^2 )
\end{equation}

where $\left\Vert \hat{h}_{j} \right\Vert = \sum_{k} \alpha_k$.  To estimate the expectation value of the full Hamiltonian \ref{eq:hamiltonian}:

\begin{equation}
    \mathcal{E} \propto \mathcal{O}( \frac{1}{\epsilon^2} \sum_{k} \Vert \alpha_k \Vert^2 \left\Vert \hat{h}_{j} \right\Vert^2 )
\end{equation}

It has been shown that in the limit p ! 1, QAOA is
capable of finding the true global optimum of the classical
combinatorial optimization problem.\cite{farhi_quantum_2017}. 

It also has important implications in computational
complexity: the ecient classical sampling of a depth-1
QAOA will collapse the polynomial hierarchy to the
third level.\cite{farhi_quantum_2019-1}

Pontryagin's maximum
principle, QAOA is optimal for solving variational
problems whose cost function is a linear function of the
system Hamiltonian.\cite{yang_optimizing_2017}

Much less is known
about QAOA performance in the low-depth (1 < p < 10)
depth regime. A recent paper [6] showed that QAOA can get CutVal Hamiltonian = Problem Hamil C + Driver Hail B
\begin{equation}
H = C + B
\end{equation}

Alternate unitary dynamics generated by C and B.\cite{farhi_quantum_2014} 
The number of alternations is denoted by p and called the depth of the QAOA circuit.


\begin{figure}
    \begin{center}\adjustimage{max size={\linewidth}{0.4\paperheight}}{figures/experiment_time-num_vertices.PNG}\end{center}
    \caption{experiment time}
    \label{fig1}
\end{figure}

\begin{figure}
    \begin{center}\adjustimage{max size={\linewidth}{0.4\paperheight}}{figures/shaydulin_multistart_2019.PNG}\end{center}
    \caption{Performance of COBYLA versus APOSMM+BOBYQA\cite{shaydulin_multistart_2019}}
    \label{fig:APOSMM}
\end{figure}

%------------------------------------------------------------------
\subsection{Cost Function}
\label{sec:VQE}
%------------------------------------------------------------------

We denote these samples by Hk(),
k = 1; : : : ;K, where K 2 N is the number of samples.
The sample mean
1
K
XK
k=1
Hk() (5)
is an estimator for h ()jH j ()i, and is used as the objective
function for the classical optimization algorithm.
The solution returned by the algorithm is then given by
the bitstring that leads to the smallest Hk among all observed
bitstrings and all  that have been evaluated.


Periodicity of the objective function with respect to QAOA
parameters, visible on heatmaps in Fig. 1, has been demonstrated
for MAXCUT,\cite{zhou_quantum_2018}.\cite{wang_quantum_2018} The periodicity was also
observed for quasi-maximum-likelihood decoding of classical
channel codes.\cite{matsumine_channel_2019} This can potentially allow for further
restriction of the domain, eliminating some of the local optima
and making the optimization problem easier. However, the
theoretical results so far are problem specific. Therefore, we
restrict our optimization domain to i 2 [0; ], 
i 2 [0; 2],
following.\cite{farhi_quantum_2014} Note that this differs from the approach in \cite{crooks_performance_2018},
where the values of  and 
 were not constrained. A recent
result shows that exploiting the periodicity of variational
parameters of certain ansatzes for QAOA and other variational
algorithms can improve optimization performance \cite{nakanishi_sequential_2019}.\cite{shaydulin_multistart_2019}



%------------------------------------------------------------------
\subsection{Circuit Depth}
%------------------------------------------------------------------

Because of NISQ, near-term algorithms require much lower circuit 
depths than algorithms with long-term Applications (e.g. 

How to construct the circuit from C (the cost function)

\begin{itemize}
\item Original Ansatz \cite{farhi_quantum_2014}
\item Considering baremetal connectivity \cite{Farhi2017a}
\item Introduce further Hamiltonians (AQO), global operations \cite{Kandala2017}
\end{itemize}


What p is required to achieved certain quality of solution?

\begin{itemize}
\item fixed p \cite{crooks_performance_2018,Guerreschi2019}
\item adapative p: linear, exp. (cite)
\end{itemize}

What is cost function we want to minimize? Ising (maxcut, maxsat, etc)

\begin{itemize}
\item $<C>$ via fixed number of samples \cite{Kandala2017,Otterbach2017a,Guerreschi2019}.
\item $<C>$ via variable number of samples, for example to keep the variance of the cost function estimate below a given threshold \cite{Guerreschi2017a}.
\end{itemize}


\begin{itemize}
\item Derivative-free like Nelder-Mean. (cite)
\item Gradient methods like BFGS, using analytical gradient \cite{Guerreschi2017a,Harrow2019a}.
\item Gradient methods using FD \cite{Guerreschi2017a}.
\item And lots of alternatives per category above.
\end{itemize}
    

%------------------------------------------------------------------
\subsubsection{Initial Values}
Circuit optimization has many local minima, how to get global?
\begin{itemize}
\item Random guesses, sequential and independent optimiation runs \cite{Guerreschi2017a}.
\item Swarm-based methods, possibility not yet explored in the literature to the best of my knowledge.
\item ML-predicted ``good values'' \cite{Wecker2016,crooks_performance_2018}
\item Optimize subset of the parameters then extend gradually to all \cite{Zhou2018a}.
\end{itemize}

%------------------------------------------------------------------
\subsubsection{Stopping Conditions}
For NP- problems, one does not know value of global solution.  When do we stop looking?
\begin{itemize}
\item Fixed number of optimization runs \cite{Guerreschi2019}
\item Fixed total WallTime (cite)
\item Convergence criteria (e.g. SGD) \cite{Guerreschi2017a}
\end{itemize}

%------------------------------------------------------------------
\section{Performance}
%------------------------------------------------------------------

WallTime + quality of solution. For maxcut, WallTime+approximation ratio.

%------------------------------------------------------------------
\subsection{Time to Solution}

\begin{itemize}

\item Define $x*$ such that $C* = C(x*)$ is the GW/MBO/etc approximate solution.

\item Run QAOA protocol (many options above) until observing sample $x$ such that $C(x) \ge  C*$. This is obtained after $s(x)$ changes of QAOA config (i.e., different set of parameter values) and a total of $t(x)$ time to execute circuits (accumulation of statistics).

\item Repeat to obtain an ensemble of $s(x)$ and $t(x)$. Compute average.

\item Notice that if p is changed during protocol, the absolute time to run a single quantum circuit depends linearly on p. 

\end{itemize}

%------------------------------------------------------------------
\begin{figure}
    \begin{center}\adjustimage{max size={\linewidth}{0.4\paperheight}}{figures/maxcut_projection.png}\end{center}
    \caption{WallTime performance}
    \label{fig1}
\end{figure}
    
\begin{figure}
    \begin{center}\adjustimage{max size={\linewidth}{0.4\paperheight}}{figures/maxcut_projection_mbo.png}\end{center}
    \caption{WallTime performance}
    \label{fig2}
\end{figure}
    
%------------------------------------------------------------------
\subsection{Qualilty of Solution}

\begin{itemize}

\item Define $x*$ such that $C* = C(x*)$ is the GW/MBO/etc approximate solution.

\item Run QAOA protocol with the stopping criteria. May require increasing p, running lots of optimization runs, etc.

\item Consider the best approximate solution from QAOA being $C^*$. Compute ratio of $C^*/C*$.

\end{itemize}

\begin{figure}
    \begin{center}\adjustimage{max size={\linewidth}{0.4\paperheight}}{figures/maxcut_bounds.png}\end{center}
    \caption{test}
    \label{fig3}
\end{figure}
    
\begin{figure}
    \begin{center}\adjustimage{max size={\linewidth}{0.4\paperheight}}{figures/maxcut_bounds_erdos_p005.png}\end{center}
    \caption{test}
    \label{fig4}
\end{figure}
    
    \begin{figure}
    \begin{center}\adjustimage{max size={\linewidth}{0.4\paperheight}}{figures/maxcut_bounds_erdos_p05.png}\end{center}
    \caption{test}
    \label{fig5}
\end{figure}
    
    \begin{figure}
    \begin{center}\adjustimage{max size={\linewidth}{0.4\paperheight}}{figures/maxcut_bounds_erdos_p10.png}\end{center}
    \caption{test}
    \label{fig6}
\end{figure}

%------------------------------------------------------------------
\subsection{Miscellaneous observations}

"To achieve this, we define a class of optimization problems with respect to their spectral properties which are exactly solvable with QAOA. In this class, we identify instances for which QA and SA have an exponentially small probability to find the solution."\cite{streif_comparison_2019}

Implications of large training budget (many circuit evaluations running in parallel over instance variation, graph types) \cite{ushijima-mwesigwa_multilevel_2019}

\begin{itemize}
    \item Recent study focused on the limitation of $p$ values by device noise \cite{alam_design-space_2020}
    \item Notes on classical performance
    \item  off-loading parameter optimization since good values can be ``recycled''. Use of CVAR approach further improves/speedups parameter optimization,\cite{barkoutsos_improving_2019} Gibb's sampling\cite{li_quantum_2020}
    \item \note{Outlook:} Machine learning for good parameter initialization?\cite{khairy_learning_2019}\cite{alam_accelerating_2020} Effect of noise: does it disrupt the under-sampling strategy? Connectivity impact on circuit duration.
\end{itemize}

It also has important implications in computational complexity: the effcient classical sampling of a depth-1 QAOA will collapse the polynomial hierarchy to the third level \cite{farhi_quantum_2019-1}.


==> old-material.tex <==
%------------------------------------------------------------------
\section{Old material to be re-arranged and updated}
\label{sec:old}
%------------------------------------------------------------------

WallTime + quality of solution. For maxcut, WallTime+approximation ratio.

%------------------------------------------------------------------
\subsection{Time to Solution}

\begin{itemize}

\item Define $x*$ such that $C* = C(x*)$ is the GW/MBO/etc approximate solution.

\item Run QAOA protocol (many options above) until observing sample $x$ such that $C(x) \ge  C*$. This is obtained after $s(x)$ changes of QAOA config (i.e., different set of parameter values) and a total of $t(x)$ time to execute circuits (accumulation of statistics).

\item Repeat to obtain an ensemble of $s(x)$ and $t(x)$. Compute average.

\item Notice that if p is changed during protocol, the absolute time to run a single quantum circuit depends linearly on p. 

\end{itemize}


\subsection{Qualilty of Solution}

\begin{itemize}

\item Define $x*$ such that $C* = C(x*)$ is the GW/MBO/etc approximate solution.

\item Run QAOA protocol with the stopping criteria. May require increasing p, running lots of optimization runs, etc.

\item Consider the best approximate solution from QAOA being $C^*$. Compute ratio of $C^*/C*$.

\end{itemize}



%------------------------------------------------------------------
\section{Comparison with classical approximate solvers}
\label{sec:comparison}
\info{This section is meant to benchmark the cost of QAOA experiments versus classical alternatives (akmaxsat for exact solvers and GW for approximate solvers).}
%------------------------------------------------------------------

\note{What about MBO?}




==> pygments-definitions.tex <==
%------------------------------------------------------------------
    % Pygments definitions
    
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother

